FDSOI Process Based MIV-transistor Utilization for Standard Cell Designs in Monolithic 3D Integration

Monolithic Three-Dimensional Integrated Circuits (M3D-IC) has become an attractive option to increase the transistor density. In M3D-IC, substrate layers are realized on top of previous layers using sequential integration techniques. Recent works in M3D-IC have demonstrated the feasibility of FDSOI process-based M3D-IC implementations and, Metal inter-layer vias (MIVs) are used to provide connections between the inter-layer devices. Since MIVs are extended from bottom layer to top layer, they occupy a small area resulting in area overhead. Additionally, a minimum separation is required to facilitate connection between MIV and transistors which increases this overhead further. Towards this, we studied the alternate utilization of MIV to create MIV-transistors with varying channels. We have also presented a strategy to extract the Spice parameters of the proposed models using level 70 spice parameters. Finally, a standard cell based gate level comparison is presented to compare the Power, Performance and Area (PPA) metrics of the traditional two layer 2D FDSOI transistor implementation with the proposed models. Simulation results from standard cell designs suggest that the proposed methodology can reduce 18\% layout area on average compared to the traditional approach. In addition, power consumption and delay time of the standard cells are reduced by 1\% and 3\% on average respectively.

==> Section3_Impact_in_FDSOI_process-backup.tex <==



%MIV (\textbf{M}etal), Buried-Oxide (\textbf{I}nsulator) and, transistor (\textbf{S}ilicon) forms an MIS structure. The terminal voltages on transistor such as Drain voltage ($V_{D}$), Source Voltage ($V_{S}$), Gate voltage ($V_{G}$), and MIV voltage ($V_{MIV}$) results in electrical coupling between the biased regions. Since the voltages can be varied in any direction, we have assumed a nominal case where $V_{MIV}=1V$ inverts the region around it.

In this section, we study the effect of MIV on nearby transistor performance in a FDSOI process of 2 layer M3D-IC. MIV (\textbf{M}etal), Buried-Oxide (\textbf{I}nsulator) and, transistor (\textbf{S}ilicon) forms an MIS structure in the top layer. The terminal voltages on transistor such as Drain voltage ($V_{D}$), Source Voltage ($V_{S}$), and Gate voltage ($V_{G}$), and other terminal voltages such as MIV voltage ($V_{MIV}$) results in electrical coupling between the biased regions.  For simplicity, we only look at a case where top layer transistors are allocated for n-type transistors. The process specifications used in the design are given Table \ref{tab:process_spec}. For this study, we look at the performance of transistor with width $w_{src}=48nm$, when MIV is placed near it as shown in Figure \ref{fig:varying_dsep_doffset_FDSOI}. The separation between MIV and transistor is denoted by $d_{sep}$. Additionally, the centers of MIV and transistors are aligned vertically. The relative shift in MIV center position compared to the center of the transistor is given by $d_{offset}$. Finally, we use a control variable method to study impact of MIV placement by varying one parameter at a given time. To evaluate the performance, we look at the leakage (Drain current, when $V_{GS}=0V$ and $V_{DS}=1V$) increase due to MIV presence compared to nominal case where MIV is absent. We assume voltage of MIV is $1V$, since it has an increased inversion effect due to the MIS structure. The findings of the study are given below:




\begin{figure*}[]
\centering
\begin{subfigure}{0.18\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Layout/FDSOI_varying_dsep.jpg}
    \caption{Layout top view}
    \label{subfig:varying_dsep_layout}
\end{subfigure}
\begin{subfigure}{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Simulation/Id_leak_change_dsep.png}
    \caption{ $ I_{D,leak}\ \% diff. $ v.s. $d_{sep}$}
    \label{subfig:varying_dsep_result}
\end{subfigure}
\begin{subfigure}{0.35\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Simulation/Id_leak_change_doffset.png}
    \caption{ $ I_{D,leak}\ \% diff. $ v.s. $d_{sep}$}
    \label{subfig:varying_doffset}
\end{subfigure}
    \caption{$I_{D,leak}$ variation due to presence of MIV near transistor}
    \label{fig:varying_dsep_doffset_FDSOI}
\end{figure*}

\subsubsection{Varying $d_{sep}$} In this case, we assume the centers are perfectly aligned ($d_{offset}=0nm$), and the separation ($d_{sep}$) is varied from $20nm$ to $200nm$. As $d_{sep}$ increased from $20nm$ to $60nm$, the change in leakage reduced significantly from $85\%$ to $20\%$. When $d_{sep}$ increased from $60nm$ to $200nm$, the change in leakage reduced slowly from $20\%$ to $10\%$. Therefore, $d_{sep}$ could be used as a metric for obtaining Keep-out-Zone (KOZ) of MIV. For example, we can consider minimum KOZ around MIV as $60nm$ based on this study to limit the leakage increase within $20\%$.  

\subsubsection{Varying $d_{offset}$} In this case, we look at the impact of offsetting the MIV position from a fixed separation and, study the impact of MIV placement on performance of transistor. To offset the MIV placement, we vary the parameter $d_{offset}$ from $-80nm$ to $+80nm$. When $d_{offset}=-80nm$, it is shifted towards the Drain (Terminal voltage is $1V$) region and, the change in leakage reduced significantly from $20\%$ to $0\%$. On the contrary, when the $d_{offset}=80nm$, it is shifted towards the Source region (Terminal voltage is $0V$) and, the change in leakage increased significantly from $20\%$ to $30\%$. This study suggests to place MIV with an offset in the center alignment towards the Drain region  to reduce the MIV effect on transistor performance. 

\textbf{Observation 1:} When MIV and the adjacent transistor gate terminal carry different voltages and are placed as shown in Figure \ref{subfig:varying_dsep_layout}, they should be separated by a minimum distance $d_{sep}$.

\textcolor{red}{Although not shown, if the MIV and the adjacent transistor carry the same voltage that is the MIV is connecting to the gate of the transistor then they can be placed as close as possible with the oxide liner around MIV and the minimum separation is not required since there is no impact of MIV on the leakage current in this scenario. We utilize this property to realize transistor wher MIV connects to the gate terminal for reducing the silicon footprint!}



%\redHL{add the connection section. KOZ, although not discussed MIV and gate terminal has same voltage dsep can be zero. and MIV transistor can be place there. Towards this end we propose MIV transistor }



\begin{figure}[]
    \centering
    \includegraphics[width=0.75\linewidth]{Figures/Simulation/Id_leak_change_dsep_horizontal.png}
    \caption{\redHL{ILD or nearby?}}
    \label{fig:unknown}
\end{figure}

